Transductive Information Maximization For Few-Shot Learning

We introduce Transductive Infomation Maximization (TIM) for few-shot learning. Our method maximizes the mutual information between the query features and their label predictions for a given few-shot task, in conjunction with a supervision loss based on the support set. Furthermore, we propose a new alternating-direction solver for our mutual-information loss, which substantially speeds up transductive-inference convergence over gradient-based optimization, while yielding similar accuracy. TIM inference is modular: it can be used on top of any base-training feature extractor. Following standard transductive few-shot settings, our comprehensive experiments demonstrate that TIM outperforms state-of-the-art methods significantly across various datasets and networks, while used on top of a fixed feature extractor trained with simple cross-entropy on the base classes, without resorting to complex meta-learning schemes. It consistently brings between 2% and 5% improvement in accuracy over the best performing method, not only on all the well-established few-shot benchmarks but also on more challenging scenarios,with domain shifts and larger numbers of classes.

==> 4_table_mini-imagenet_CUB.tex <==
\begin{table}
    \centering
    \begin{tabular}{lcccccccc}
        & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{CUB}}} & \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}{c}\textbf{\textit{mini}-ImageNet}\\ \textbf{to CUB}\end{tabular}}} & \multicolumn{4}{c}{\textbf{\textit{mini}-ImageNet}} \\
        & & & & & \multicolumn{2}{c}{10-way} & \multicolumn{2}{c}{20-way} \\
        Method & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot & 1-shot & 5-shot\\
        \toprule
        MatchNet \cite{matching_net} &  73.5 & 84.5 & - & 53.1 & - & 52.3 & - & 36.8 \\
        MAML \cite{maml} & 68.4 & 83.5 & - & 51.3 & - & - & - & - \\
        ProtoNet \cite{prototypical_nets} & 73.0 & 86.6 & - & 62.0 & - & 59.2 & - & 45.0 \\
        RelatNet \cite{relation_net} & 68.6 & 84.0 & - & 57.7 & - & 53.9 & - & 39.2 \\
        CL2N \cite{simpleshot} & 68.9 & 84.0 & 48.0 & 64.0 & 45.1 & 68.1 & 32.4 & 55.4 \\
        Baseline \cite{closer_look} & 65.5 & 82.9 & - & 65.6 & - & 55.0 & - & 42.0 \\
        Baseline++ \cite{closer_look} & 67.0 & 83.6 & - & 62.0 & - & 63.4 & - & 50.9 \\
        \rowcolor{Gray} TIM-ADM & \textbf{79.2} & 86.2 & 51.2 & 65.6 & 52.1 & 69.1 & 33.5 & 53.8 \\
        \rowcolor{Gray} TIM-GD & 79.0 & \textbf{87.6} & \textbf{54.4} & \textbf{71.0} & \textbf{55.6} & \textbf{72.2} & \textbf{39.4} & \textbf{59.0} \\
        \bottomrule
    \end{tabular}
    \caption{Results for CUB, domain-shift \textit{mini}-Imagenet $\rightarrow$ CUB and increased ways on \textit{mini}-ImageNet with a ResNet-18 architecture. Our results (gray-shaded) are averaged over 10,000 episodes.}
    \label{tab:domin_shift_increased_results}
\end{table}


